JAILJUDGE: A Comprehensive Jailbreak Judge Benchmark with Multi-Agent Enhanced Explanation Evaluation Framework

Despite advancements in enhancing LLM safety against jailbreak attacks, evaluating LLM defenses remains a challenge, with current methods often lacking explainability and generalization to complex scenarios, leading to incomplete assessments (e.g., direct judgment without reasoning, low F1 score of GPT-4 in complex cases, bias in multilingual scenarios). To address this, we present JAILJUDGE, a comprehensive benchmark featuring diverse risk scenarios, including synthetic, adversarial, in-the-wild, and multilingual prompts, along with high-quality human-annotated datasets. The JAILJUDGE dataset includes over 35k+ instruction-tune data with reasoning explainability and JAILJUDGETEST, a 4.5k+ labeled set for risk scenarios, and a 6k+ multilingual set across ten languages. To enhance evaluation with explicit reasoning, we propose the JailJudge MultiAgent framework, which enables explainable, fine-grained scoring (1 to 10). This framework supports the construction of instruction-tuning ground truth and facilitates the development of JAILJUDGE Guard, an end-to-end judge model that provides reasoning and eliminates API costs. Additionally, we introduce JailBoost, an attacker-agnostic attack enhancer, and GuardShield, a moderation defense, both leveraging JAILJUDGE Guard. Our experiments demonstrate the state-of-the-art performance of JailJudge methods (JailJudge MultiAgent, JAILJUDGE Guard) across diverse models (e.g., GPT-4, Llama-Guard) and zero-shot scenarios. JailBoost and GuardShield significantly improve jailbreak attack and defense tasks under zero-shot settings, with JailBoost enhancing performance by 29.24% and GuardShield reducing defense ASR from 40.46% to 0.15%.

==> tabs/judge_as_def.tex <==
\begin{table}[tbp]
    \centering
    \caption{JAILJUDGE as the defense method. }
    \small
    \label{tab:judge_def}
    \resizebox{\textwidth}{!}{
    \begin{tabular}{lcccc}
        \toprule
        \textbf{Defense Methods} & \textbf{AutoDAN}$\downarrow$ & \textbf{PAIR}$\downarrow$ & \textbf{AdvPrompter}$\downarrow$ & \textbf{AmpleGCG}$\downarrow$ \\ 
        \midrule
    
        No Defense & 69.39 & 40.61 & 37.27 & 14.85 \\
        Self-Reminder & 36.36 & 31.82 & 10.91 & 8.18 \\
        RPO & 46.06 & 34.24 & 0.91 & 0.30 \\
        Unlearn & 66.06 & 52.12 & 45.45 & 30.00 \\
        Adv. Training & 41.82 & 30.30 & 28.79 & 2.73 \\
        ShieldGemma-9B & 9.09 & 8.48 & 10.00 & 6.36 \\
        Llama-Guard-3-8B & \textbf{0.00} & \textbf{0.00} & \textbf{0.00} & \textbf{0.00} \\
        GuardShield (Ours) & \textbf{0.00} & \underline{0.61} & \textbf{0.00} & \textbf{0.00} \\
        \bottomrule
\end{tabular}
}
\end{table}

